Bridging the Gap Between Value and Policy Based Reinforcement Learning

We establish a new connection between value and policy based reinforcement learning (RL) based on a relationship between softmax temporal value consistency and policy optimality under entropy regularization. Specifically, we show that softmax consistent action values correspond to optimal entropy regularized policy probabilities along any action sequence, regardless of provenance. From this observation, we develop a new RL algorithm, Path Consistency Learning (PCL), that minimizes a notion of soft consistency error along multi-step action sequences extracted from both on- and off-policy traces. We examine the behavior of PCL in different scenarios and show that PCL can be interpreted as generalizing both actor-critic and Q-learning algorithms. We subsequently deepen the relationship by showing how a single model can be used to represent both a policy and the corresponding softmax state values, eliminating the need for a separate critic. The experimental evaluation demonstrates that PCL significantly outperforms strong actor-critic and Q-learning baselines across several benchmarks.

==> background.tex <==
\section{Background}
First, consider the
standard
expected reward objective:
\begin{eqnarray}
  \mro(\pi, s) &=& \sum_a \pi(a \mid s)\,\sum_{s', r} p(s', r \mid s, a)\,[r(s, a) + \gamma \vop(s')]\\
   &=& \sum_a \pi(a \mid s)\,\expected_{(s',\,r)}\,[r(s, a) + \gamma \vop(s')]~.
\end{eqnarray}

\begin{eqnarray}
  \label{eq:hard2} \vop(s) ~=~ \mro(\piop, s) &=& \max_{a} \sum_{s', r} p(s', r \mid s, a)\,[r(s, a) + \gamma \vop(s')]\\
&=& \max_{a} \,\expected_{(s',\,r)}\,[r(s, a) + \gamma \vop(s')]~.
\end{eqnarray}

\begin{equation}
  \ento(\pi, s, \temp) ~=~ \sum_a \pi(a \mid s)\,\expected_{(s',\,r)}\,
       [r + \gamma \Vstar(s') - \temp \log\pi(a\mid s)]~,
\end{equation}

\begin{equation}
\Vstar(s) = \ento(\pistar, s, \temp) = \tau\log \sum_a \exp\{\,\expected_{(s',\,r)}\,[r + \gamma
\Vstar(s')]/\tau\,\}
.
\label{eq:vsimple}
\end{equation}




\section{Background}
\label{background}
Our method uses a softmax temporal consistency 
to establish a connection between
value and policy based RL.  
The literature currently considers two primary notions of temporal consistency,
which we refer to as {\em average} \eqref{eq:avg} and 
{\em hard-max} \eqref{eq:hard} consistency respectively:
\begin{eqnarray}
\label{eq:avg}  \qpi(s, a) &=& r(s, a) + \gamma\expected_{\pi(a^\prime|s^\prime)} \qpi(s^\prime, a^\prime)~,\\
\label{eq:hard}  \qop(s, a) &=& r(s, a) + \gamma\max_{a'} \qop(s^\prime, a')
~,
\end{eqnarray}
where a state action pair $(s, a)$ is followed by
a state $s'$ and $0 \leq \gamma \leq 1$ is the reward {\em discount} factor.  
One may equivalently express these consistencies in terms state value functions,
defined for the expected and hard-max cases respectively as
\begin{eqnarray}
\label{eq:avg2} \vpi(s) &=& \expected_{\pi(a|s)} [r(s, a) + \gamma \vpi(s')]~,\\
\label{eq:hard2} \vop(s) &=& \max_{a} (r(s, a) + \gamma \vop(s'))~.
\end{eqnarray}

The constraint in~\eqref{eq:avg} and~\eqref{eq:avg2} 
applies to any policy $\pi$ 
and serves as the basis of the {\em on-policy} one-step expected
SARSA~~\cite{rummery1994,singh1996} 
and multi-step actor-critic~\cite{mnih2016asynchronous} algorithms;
while the constraint in~\eqref{eq:hard} and~\eqref{eq:hard2}
only applies to a maximum reward policy
and is the basis of the {\em off-policy} Q-learning algorithm~\cite{qlearning}.

\comment{
In particular,
the actor-critic algorithm~\citep{mnih2016asynchronous} maintains an
estimate of $\vpi$ to estimate the future expected rewards beyond a
certain state.  This allows for estimating the value of one or several
actions without rolling out an entire trajectory until
termination. 
In addition,
$\vpi$ is used as a baseline to reduce the
variance of gradients.

The Q-learning algorithm~\citep{qlearning} exploits the fact that the 
hard-max consistent Q-values, denoted $\qop$, induce a policy with
maximal expected reward, where at each state $s$ one chooses an
action with largest $\qop(s, a)$. 
The Q-learning algorithm then minimizes one-step hard-max 
inconsistencies induced by a Q-value approximator $\Qphi(s, a)$.
}


==> intro2.tex <==
\comment{
\section{Softmax Temporal Consistency}

{\color{red} Kelvin: Should this be in the preliminaries?}
At iteration $t$, the agent encounters a state $\s_t$, performs
an action $\a_t$, and the environment returns a scalar reward $r_t$,
moving to the next state $\s_{t+1}$.

% Think of a better way to motivate deterministic environments
To simplify matters, this paper focuses on deterministic environments
for which the transition from $(\s, \a)$ to $\s'$ is deterministic,
\eg~$\s' = f(\s, \a)$. We expect our results to generalize to
stochastic environments, but we leave that to future
work. There exist two types of temporal consistency for action values
in the literature, which we call {\em average} consistency in
\eqref{eq:avg} below and {\em hard-max} consistency in
\eqref{eq:hard},
\begin{eqnarray}
\label{eq:avg}  \qpi(s, a) &=& r(s, a) + \gamma\expected_{\pi(a^\prime|s^\prime)} \qpi(s^\prime, a^\prime)~,\\
\label{eq:hard}  \qop(s, a) &=& r(s, a) + \gamma\max_{a'} \qop(s^\prime, a')~,
\end{eqnarray}
where $0 \leq \gamma \leq 1$ is the reward {\em discount} factor.  The
former constraint is the basis for the {\em on-policy} one-step
expected SARSA algorithm, and the latter is used within the {\em
  off-policy} Q-learning algorithm. In both cases, the so-called {\em
  Bellman} operators~\cite{bellman1957} on the RHS of \eqref{eq:avg}
and \eqref{eq:hard} are used to improve the estimates of the Q
values on the LHS by one-step bootstrapping.

Despite the common observation that entropy regularization improves
the empirical behavior of RL
algorithms~\cite{williams1991function,mnih2016asynchronous,urex},
recent methods still rely on average~\eqref{eq:avg} or
hard-max~\eqref{eq:hard} backups that are associated with an expected
reward objective with no regularization.  In this paper, we propose a
novel {\em softmax}\footnote{In this paper, the term {\em softmax}
  refers to a log-sum-exp function and the term {\em soft indmax}
  refers to the normalized exponential function or so-called softmax
  activation function, which produces a multinomial distribution.}
temporal consistency that takes regularization into account:
\begin{equation}
\label{eq:soft}
  \qs(s, a) ~=~ r(s, a) + \gamma\tau \log\sum_{a^\prime} \exp(\qs(s^\prime, a^\prime) / \tau)~,
\end{equation}
where $\temp$ controls the strength of entropy regularization.
The softmax consistency generalizes~\eqref{eq:hard} because in the
limit, as $\temp$ approaches $0$, the log-sum-exp operator approaches
a hard max, and we are back to one-hot optimal policy in the absence
of regularization.

We prove that the softmax Bellman operator \eqref{eq:soft} is a
contraction map with a unique fixed point at the optimal policy
$\pi^*$ of the regularized expected reward. Moreover, we formulate
multi-step softmax temporal consistency that relates the Q values that
are multiple steps apart on any path with the log probabilities of
$\pi^*$ on the edges of the path. The multi-step softmax consistency
is degenerate for the case of hard-max, \ie~$\temp=0$, which explains
why multi-step Q-learning is not well defined \todo{true?}

The two common definitions of state-action Q-values $\qpi,\qop$
have already been introduced in~\eqref{eq:avg},~\eqref{eq:hard}.
Instead of state-action values, it is often cleaner to refer to 
state value functions.  The expected state value and the hard-max state 
value are defined as
\begin{eqnarray}
\vpi(s) &=& \expected_{\pi(a|s)} \qpi(s, a)~,\\
\vop(s) &=& \max_{a} \qop(s, a)~.
\end{eqnarray}
% while the soft-max value is given by 
% \begin{equation}
% \label{eq:vstar}
% \vstar(s) ~=~ \tau \log\sum_{a} \exp(\qs(s, a) / \tau)~.
% \end{equation}
The expected value function $\vpi$ is used in SARSA
and actor-critic algorithms
while the hard-max value function $\vop$ is the basis for Q-learning
and its many successful variants.  
Our proposed algorithm is most similar to 
actor-critic and Q-learning,
so we provide a brief overview of each.


As the expected and hard-max Q-values
have natural definitions of state value functions,
so do the soft-max Q-values.  We 
define the soft-max state value function as
\begin{equation}
\label{eq:vstar}
\vstar(s) ~=~ \tau \log\sum_{a} \exp(\qs(s, a) / \tau)~.
\end{equation}
While the hard-max $\qop,\vop$ share 
an intimate relationship with the optimal policy
under the maximum reward objective $O_{MR}$,
we show that $\qs,\vstar$ are intimately related 
to the optimal policy under an entropy-regularized
maximum reward objective.
}


==> intro_old.tex <==

\comment{ %%%%%%

\section{Introduction}
\label{intro}

Model-free RL aims 
to acquire an effective behavior policy through 
trial and error
interaction with a black box environment. % via trial and error.
The goal is to optimize the quality of an agent's behavior policy,
in terms of the total expected discounted reward.
Model-free RL has a myriad of
applications in games~\cite{tesauro1995,atarinature},
robotics~\cite{kober2013,levine2016end},
and marketing~\cite{li2010,theocharous2015}, to name a few.

The two dominant approaches to developing model-free RL 
algorithms 
%include 
have been
{\em value based} and {\em policy based}. 

} %%%%%%% end comment

Although these approaches have typically been considered distinct,
recent work \cite{rml2016,pgq2017} has begun to relate the two
by posing {\em entropy regularized} expected reward as the 
target objective~\cite{williams1991function}. 
Given entropy regularization, the optimal policy $\pistar$ assigns a probability to an action
sequence that is proportional to the exponentiated 
total reward received. %  along each sequence of states and actions.
In particular, given an episode of states, 
actions and rewards, $(s_0,a_0,r_0,\ldots,s_{T-1},a_{T-1},r_{T-1},s_T)$, 
where $s_T$ is a terminal state, 
the optimal policy $\pistar$ satisfies,
%\vspace{-2mm}
\begin{equation}
  \prod\nolimits_{i=0}^{T-1} \pistar(a_i\mid s_i) 
\propto 
\exp \Big( \sum\nolimits_{i=0}^{T-1} r_i / \temp \Big)~,
  \label{eq:opt-policy}
\end{equation}
%\vspace{-5mm}
where $\temp \geq 0$ is an entropy regularization coefficient.
Unfortunately, such results have only been established 
thus far 
%to this point
for undiscounted finite horizon tasks.

This paper further develops a connection between value and policy based RL
by considering a notion of temporal difference consistency in 
the presence of {\em discounted} entropy regularization,
which not only allows extension to the infinite horizon case,
but also reveals surprisingly strong new properties.
Consider a transition where a state action pair $(s, a)$ is followed by%
%
\footnote{
To simplify matters, we focus on environments with a 
\emph{deterministic} transition from $(s, a)$ to $s'$. 
Such transitions may depend on a shared random seed,
applicable to a wide range of tasks.
} 
a state $s'$.
The literature currently considers two primary notions of temporal consistency,
which we refer to as {\em average} \eqref{eq:avg} and 
{\em hard-max} \eqref{eq:hard} consistency respectively:
%\vspace{-2mm}
\begin{eqnarray}
\label{eq:avg}  \qpi(s, a) &=& r(s, a) + \gamma\expected_{\pi(a^\prime|s^\prime)} \qpi(s^\prime, a^\prime)~,\\
\label{eq:hard}  \qop(s, a) &=& r(s, a) + \gamma\max_{a'} \qop(s^\prime, a')
~.
\end{eqnarray}
%\vspace{-5mm}
Here $0 \leq \gamma \leq 1$ is the reward {\em discount} factor.  
The constraint \eqref{eq:avg} applies to any policy $\pi$ 
and serves as the basis of the {\em on-policy} one-step expected
SARSA~~\cite{rummery1994,singh1996} 
and actor-critic~\cite{mnih2016asynchronous} algorithms;
while the constraint~\eqref{eq:hard} only applies to a maximum reward policy
and is the basis of the {\em off-policy} Q-learning algorithm~\cite{qlearning}.

Given $\gamma$-discounted entropy regularization, 
we formulate a new notion of {\em softmax}
temporal consistency for optimal Q-values as:
%
\begin{equation}
\label{eq:soft}
 \qs(s, a) = r(s, a) + \gamma\tau \log\sum\nolimits_{a^\prime} 
\exp(\qs(s^\prime, a^\prime) / \tau)~.
\end{equation}
%
Note that as $\temp\!\rightarrow\!0$ the standard hard-max consistency
\eqref{eq:hard} is recovered as a special case. 
%
For finite action spaces and discrete state spaces, given a deterministic
state transition function,
we prove that a {\em unique} solution $\qs$ 
to the softmax consistency constraint \eqref{eq:soft} must exist. 
Further, we show that the policy
$\pistar(a \mid s) \propto \exp(\qs(s, a)/\temp)$ %built on 
defined from
$\qs$ %values
maximizes entropy regularized expected discounted reward.
Crucially,
%we extend 
this notion of softmax %temporal 
consistency 
can be extended
beyond single step backups
to derive multi-step path-wise consistency constraints
\emph{on arbitrary trajectories},
in contrast to the standard hard-max consistency \eqref{eq:hard}.
%% Mo: Improve sentence above -- why is there a contrast?

%% , in which $\pistar(s, a)$ being proportional to exponentiated Q-values

%% Utilizing these path-wise consistencies,

\comment{ %%%%%%%

Based on these developments, we propose a new RL algorithm,
\emph{\longname (\shortname)},
that optimizes a policy by minimizing the path-wise temporal
inconsistency on a set of on and off policy traces.  \shortname
iteratively fits both a parameterized policy and a state value
function (implicitly Q-values), bridging the gap between value and
policy based methods.  
Unlike algorithms using $\qpi$-values, 
the proposed approach seamlessly combines on-policy and off-policy traces.  
Unlike algorithms based on hard-max consistency and $\qop$-values, 
the proposed formulation easily generalizes to multi-step backups 
on arbitrary paths,
while maintaining proper regularization and 
consistent mathematical justification. 
We assess the effectiveness of \shortname on a suite of RL benchmarks,
and we find that it significantly outperforms a strong
actor-critic and a strong Q-learning baseline.

In summary, the main contributions of this paper include:
\vspace{-.4cm}
\begin{itemize}
  \setlength{\parskip}{0pt}
  \setlength{\itemsep}{0pt plus 1pt}
    \item A complete characterization of 
%A new 
{\em softmax} temporal consistency,%
%
\footnote{
We use the term {\em softmax} to refer to the log-sum-exp function,
and {\em soft indmax} to refer to the normalized exponential function 
corresponding to the (regrettably misnamed) ``softmax activation function''
that produces a vector of multinomial probabilities.
} which generalizes
      the commonly used hard-max Bellman consistency.
    \item A proof that Q-values satisfying softmax temporal
      consistency directly determine the optimal policy 
      that maximizes entropy regularized expected discounted reward.
    \item Identification of a new multi-step {\em path-wise} softmax consistency property that
      relates the optimal Q-values at the end points of \emph{any path} to
      the log-probabilities of the optimal policy along actions of that path.
    \item An effective RL algorithm, \longname, that exploits
      multi-step path-wise consistency and combines elements of value and
      policy based RL.%
    \item Strong experimental results versus current actor-critic and Q-learning baselines.
\end{itemize}
\vspace{-.4cm}
%
} %%%%%%% end comment

